An observation of the $f_0(1710)$ meson in the $\omega\phi$ system in the Pion-$Be$ Interaction at Momentum of 29 GeV

The charge-exchange reaction $\pi^-p \rightarrow n\,\omega(783)\phi(1020)$, $\omega \rightarrow \pi^+\pi^-\pi^0$, $\phi \rightarrow K^+K^-$ is studied with the upgraded VES facility (U-70, Protvino) in the interaction of a 29 GeV pion beam with a beryllium target. The distribution over the invariant mass of the system $M_{\omega\phi}$ shows a near-threshold signal. A partial wave analysis reveals that the scalar state ($J^{PC}=0^{++}$) dominates in this mass region. The observed signal can be described with a contribution of the known resonance $f_0(1710)$. Using OPE approximation for the reaction $\pi^-p \rightarrow n\, f_0(1710)$ the product of branching fractions is found to be: $Br(f_0(1710)\rightarrow \pi\pi)\cdot Br(f_0(1710)\rightarrow \omega\phi) = (4.8 \pm 1.2) \cdot 10^{-3}$.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} Amelin et al., Phys.Phys.Atom.Nucl. 69 (2006) 6, 715


\end{thebibliography}


